Non-smooth Bayesian Optimization in Tuning Problems

Building surrogate models is one common approach when we attempt to learn unknown black-box functions. Bayesian optimization provides a framework which allows us to build surrogate models based on sequential samples drawn from the function and find the optimum. Tuning algorithmic parameters to optimize the performance of large, complicated "black-box" application codes is a specific important application, which aims at finding the optima of black-box functions. Within the Bayesian optimization framework, the Gaussian process model produces smooth or continuous sample paths. However, the black-box function in the tuning problem is often non-smooth. This difficult tuning problem is worsened by the fact that we usually have limited sequential samples from the black-box function. Motivated by these issues encountered in tuning, we propose a novel additive Gaussian process model called clustered Gaussian process (cGP), where the additive components are induced by clustering. In the examples we studied, the performance can be improved by as much as 90% among repetitive experiments. By using this surrogate model, we want to capture the non-smoothness of the black-box function. In addition to an algorithm for constructing this model, we also apply the model to several artificial and real applications to evaluate it.

==> Cover.tex <==
September 13, 2021
Dear Editor,
I submit the manuscript “Non-smooth Bayesian Optimization in Tuning Problems” for scrutiny and review by the editors of Journal of Machine Learning Research (JMLR), on behalf of the co-authors with their full consent and confirmation. 
To our best knowledge, this work has no significant overlapping with any of our previous research papers. We declare that we have no conflict of interest with other funding sources except for the funding disclosed in acknowledgment, institution or individuals. None of the authors of this paper is in collaborative relationship with any action editors of JMLR. Based on the focus of this paper, we suggest that the following action editors of JMLR will be suitable for reviewing our paper: Dr. Francesco Orabona,  Dr. Peter Auer, Dr. Sebastien Bubeck.
Applied and methodological studies have shown the difficulty in fitting a Gaussian regression model for unknown “black-box functions” in Bayesian optimization when non-smoothness exists. Earlier works have not addressed this problem systematically in the surrogate-base optimization. On the one hand, Gaussian regression is widely used in Bayesian optimization but has smooth sample paths; on the other hand, tuning problems often have non-smooth features and relatively many parameters under quite limited sampling budget. We combine the strength of additive model and our novel cluster-classify step for component creation, coming up with an innovative methodology to use additive Gaussian models with sequential samples within Bayesian optimization framework, to detect and model non-smoothness in the “black-box” function. We called this model the clustered Gaussian process model (cGP).  
Our approach is based on Bayesian additive models and, in particular, take both input (x) and response (y) together in the cluster-classify step for each sequential sampling phase. We formalize our model in a Bayesian framework, with theoretically justified weighted sampling algorithms. We also highlight the detecting and optimization performance of this cGP method by providing simulation studies and real data analysis on high-performance computation clusters to show that the cGP surrogate model performs surprisingly well compare to typical GP surrogate used in the Bayesian optimization. 
We believe that this manuscript perfectly fits the scope of the Journal of Machine Learning Research that it publicizes new principled algorithms with sound empirical validation and justification of theoretical nature. We propose a brand-new model called clustered Gaussian Process (cGP) which detects non-smoothness in the “black-box” function in an online surrogate-based optimization setting. Our innovative methodology applies well to both synthetic and real datasets. Overall, we believe that our manuscript provides a significant innovation on modeling non-smoothness with additive Gaussian process regression and enhance the Bayesian optimization in scientific computation tuning context.
For these reasons, I hope that the manuscript will be considered for publication in JMLR.
Sincerely,
Hengrui Luo
Computational Research Department, SSG,
Lawrence Berkeley National Laboratory,
Berkeley, CA, 94701

==> Non-smooth Bayesian Optimization in Tuning Problems_arXiv/Cover.tex <==
September 13, 2021
Dear Editor,
I submit the manuscript “Non-smooth Bayesian Optimization in Tuning Problems” for scrutiny and review by the editors of Journal of Machine Learning Research (JMLR), on behalf of the co-authors with their full consent and confirmation. 
To our best knowledge, this work has no significant overlapping with any of our previous research papers. We declare that we have no conflict of interest with other funding sources except for the funding disclosed in acknowledgment, institution or individuals. None of the authors of this paper is in collaborative relationship with any action editors of JMLR. Based on the focus of this paper, we suggest that the following action editors of JMLR will be suitable for reviewing our paper: Dr. Francesco Orabona,  Dr. Peter Auer, Dr. Sebastien Bubeck.
Applied and methodological studies have shown the difficulty in fitting a Gaussian regression model for unknown “black-box functions” in Bayesian optimization when non-smoothness exists. Earlier works have not addressed this problem systematically in the surrogate-base optimization. On the one hand, Gaussian regression is widely used in Bayesian optimization but has smooth sample paths; on the other hand, tuning problems often have non-smooth features and relatively many parameters under quite limited sampling budget. We combine the strength of additive model and our novel cluster-classify step for component creation, coming up with an innovative methodology to use additive Gaussian models with sequential samples within Bayesian optimization framework, to detect and model non-smoothness in the “black-box” function. We called this model the clustered Gaussian process model (cGP).  
Our approach is based on Bayesian additive models and, in particular, take both input (x) and response (y) together in the cluster-classify step for each sequential sampling phase. We formalize our model in a Bayesian framework, with theoretically justified weighted sampling algorithms. We also highlight the detecting and optimization performance of this cGP method by providing simulation studies and real data analysis on high-performance computation clusters to show that the cGP surrogate model performs surprisingly well compare to typical GP surrogate used in the Bayesian optimization. 
We believe that this manuscript perfectly fits the scope of the Journal of Machine Learning Research that it publicizes new principled algorithms with sound empirical validation and justification of theoretical nature. We propose a brand-new model called clustered Gaussian Process (cGP) which detects non-smoothness in the “black-box” function in an online surrogate-based optimization setting. Our innovative methodology applies well to both synthetic and real datasets. Overall, we believe that our manuscript provides a significant innovation on modeling non-smoothness with additive Gaussian process regression and enhance the Bayesian optimization in scientific computation tuning context.
For these reasons, I hope that the manuscript will be considered for publication in JMLR.
Sincerely,
Hengrui Luo
Computational Research Department, SSG,
Lawrence Berkeley National Laboratory,
Berkeley, CA, 94701
